Operationalizing AI in Future Networks: A Bird's Eye View from the System Perspective

Modern Artificial Intelligence (AI) technologies, led by Machine Learning (ML), have gained unprecedented momentum over the past decade. Following this wave of "AI summer", the network research community has also embraced AI/ML algorithms to address many problems related to network operations and management. However, compared to their counterparts in other domains, most ML-based solutions have yet to receive large-scale deployment due to insufficient maturity for production settings. This article concentrates on the practical issues of developing and operating ML-based solutions in real networks. Specifically, we enumerate the key factors hindering the integration of AI/ML in real networks and review existing solutions to uncover the missing considerations. Further, we highlight a promising direction, i.e., Machine Learning Operations (MLOps), that can close the gap. We believe this paper spotlights the system-related considerations on implementing \& maintaining ML-based solutions and invigorate their full adoption in future networks.

==> case_study.tex <==
\iffalse
**************reviewer 3***********************
\footnote{\textcolor{pink}{reviewer 3: However, the major weakness of the paper is that it focuses more on supervised learning. In particular, presenting only one use-case that leverages supervised learning is the shortcoming of the study. Considering that computer networks are highly dynamic and unpredictable, unsupervised and reinforcement learning based use cases should also be presented in the study.
}}
**************reviewer 3***********************
\fi


This section demonstrates the benefits of MLOps with two case studies on a real network benchmark. Specifically, we implement an ML-based solution for KPI forecasting, a crucial task for predictive maintenance in operational networks. To retain production setting, we deploy software network services across a distributed cluster inside a small-scale enterprise data center, where each node is a commodity off-the-shelf server equipped with Intel$^{\tiny{\textregistered}}$ Xeon CPUs and Intel$^{\tiny{\textregistered}}$ 10/40-Gigabit network cards. 
The network services attain line-rate traffic processing. 

\subsubsection*{Use cases definition}

We predict the overall network service performance, e.g., throughput, using the features of the underlying hardware subsystems, including Processor, Memory, and PCI buses, to circumvent the intricacy of in-band data collection. These features can be readily obtained using standard profiling tools. As detailed in \cite{manousis2020contention}, though these features seem less relevant than the packet-/flow-level statistics, they contain valuable insights on service performance and can be utilized for KPI predictions. To elude the aforementioned manual exertions throughout the data preparation, development, and operations phases, we adopt common MLOps practices to build a prototypical data processing pipeline, whose workflow is detailed as follows:

\begin{itemize}
\item Data preparation: We define standard procedures for the entailed steps (i.e., data collection, validation, and labeling) to automatically obtain high-quality data without interfering with the normal operations in the data plane. %By continuously monitoring CPU data and analyzing it for signs of throughput deviation, MLOps can automatically detect changes in data patterns, signaling potential shifts in network conditions or input distributions.  
\item Feature selection: To extract the most relevant features from the $\sim$600 features collected by standard profiling tools (e.g., Linux perf, Intel PCM), we employ Pearson's correlation coefficient to assay their statistical dependencies with the target service KPIs. 
\item Automated model selection: According to the studies of Manousis et al.~\cite{manousis2020contention}, we consider three ML models: Linear Regression, Gradient Boosting Regression, and Artificial Neural Network, for automated model selection. 
\item Automated hyper-parameter tuning: We employ Bayesian optimization to evaluate the performance of different hyperparameter combinations and build a probabilistic model to automatically select the optimal one. 
\item Performance monitoring and feedback loop: We employ the Jensen-Shannon divergence to inspect the input data distribution to establish a continuous monitoring mechanism. When the new data diverges from the training data, the feedback loop should be activated to retrain and roll out an up-to-date model. \textcolor[HTML]{006400}{ Accuracy metrics rely on comparing predictions to actual labels, a challenge in production due to delayed or inaccessible labels. Monitoring changes in input distributions offers an alternative when direct label comparison isn't feasible.}
%\item Model retraining and deployment: MLOps facilitates automated model retraining in response to data drifts. This retraining is triggered based on predefined criteria, ensuring the model remains up-to-date with the network status. 
\item Versioning and experiment tracking: we employ MLflow~\cite{databricks} to maintain detailed records of all the involved model artifacts, datasets, (hyper-)parameters, and other assets in the model development process, ensuring both reproducibility and auditability. %, which is crucial for ascertaining model performance over time.  %and for auditing purposes.
%\item CI/CD: Implement CI/CD pipelines for the ML models, similar to software development practices. This ensures seamless and automated testing and deployment of updated models to the system environment.
\end{itemize}





\subsubsection*{Experimental results}
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/usercase_illustration.pdf}
    \caption{The MLOps benefits on accuracy and efficiency. \textcolor{red}{execution time}.}
    \label{fig:accuracy_improvement}
\end{figure}

\footnote{\textcolor{blue}{reviewer2: The results figure, i.e., Figure 4, does not identify the baseline for the percentages, nor is this information apparent from the text.}}
An empirical evaluation of our data processing pipeline is presented in Fig.~\ref{fig:accuracy_improvement}. We focus on two test scenarios: a singleton virtual network function (L2 bridge) and a Linear Service Chain (SFC) with five network functions. For each scenario, we collect the training data under varied input loads. We first investigate the benefits of incrementally applying the customized data preparation, feature selection, model selection, and hyper-parameter tuning procedures. As shown in Fig.~\ref{fig:accuracy_improvement}, our systematic refinement strategies can incrementally enhance the overall accuracy, i.e., $76\% \rightarrow 96\%$ for bridge and $62\% \rightarrow 84\%$ for SFC. Furthermore, the implemented automation can significantly reduce the incurred model delivery time compared to the conventional, manual approaches. In particular, the time required to detect data drift has been reduced to merely $0.4$ seconds, thanks to the seamless identification of distribution shifts. Given that our prototype has not even integrated the most advanced tools and techniques, we believe MLOps can offer huge performance boosts and smooth the adoption of AI/ML in future networks. \footnote{\textcolor{red}{Reviewer 1 mentioned, Why only accuracy and efficiency has been considered as a parameter for study? What comprises efficiency? }}

\footnote{\textcolor{red}{Reviewer 1 mentioned, The present work fails to achieve the objectives as identified. The authors intention to verify the claims made in the paper have not been backed by substantial proof and rigor. }}


==> introduction.tex <==
\section*{Introduction}
\textcolor{orange}{To drive digital transformation, modern telecommunication networks are undergoing a disruptive evolution. The ongoing 5G rollout promises to deliver customized network services to billions of subscribers with ultra-high speed, ultra-high reliability, ultra-low latency, and ubiquitous connectivity. The massification of Internet-of-Things is expected to connect trillions of devices and create brand-new business models. Next-generation digital realms, e.g., Metaverse, also call for high-quality, customizable communication mediums to drive human-machine interaction and digital-physical fusion. These technical headways inevitably make modern networks increasingly diverse, decentralized, and complex. Traditionally, networks were mainly managed by predefined or \textcolor[HTML]{006400}{ad-hoc rules-- temporary and spontaneously solution adaptable for specific issues as they arise.}
\iffalse
**************reviewer 2*********
%\footnote{\textcolor{blue}{Reviewer2 : It is not readily evident what "ad-hoc rules" means in the first paragraph of the Introduction. Elaboration is required lest the term be misunderstood.}}.
**************reviewer 2*********
\fi
However, these methods either bear oversimplified assumptions about the underlying systems or incur huge computation overhead, which disaccords with the continuing network complexification.}
%{\color{red}Although the transition towards network softwarization can significantly reduce operational overhead, the programmable network infrastructures further expand the network management boundaries, leading to new issues and challenges.} 
As of today, human participation is still essential for in-depth problem diagnoses and decision-making.\footnote{\textcolor{red}{changeable, Reviewer 1 do not like this sentence.}}
\footnote{\textcolor{blue}{Reviewer 1 opinion: The authors claim that the ‘paper aspires to elucidate the practical challenges of integrating AI/ML into the future network landscape’, however, the discussion presented by the authors lack sufficient proof and analysis. It seems the authors have tried to cover a large number of points but have failed to substantiate the claims with sufficient results and outcomes.} $\rightarrow$: maybe we can start/strict introduction directly in the field of high-speed networks/virtual networks. }

\textcolor{orange}{With the accruing breakthroughs over the last decade, modern AI/ML has achieved human-level performance in many challenging tasks, e.g., computer vision, gaming, and, more recently, natural language processing. Nowadays, AI/ML-empowered products have permeated various industrial and business sectors, including healthcare, manufacturing, entertainment, and education.}\footnote{\textcolor{red}{changeable, Reviewer 1 does not like this sentence. }} According to the findings of Gartner and MIT Sloan Management Review, AI has led to \$3.9T of business value in 2022 and is deemed a strategic priority by 83\% of CEOs~\cite{databricks}. Inspired by these successes, network researchers are extensively exploring AI/ML algorithms for network automation and management. This new breed of {\em ML-based networking solutions}\footnote{Note that we focus on the data-driven branch of AI techniques, frequently denoted as ML. By abuse of language, we will use the two acronyms interchangeably in this paper.}, i.e., applications, functions, and services, have demonstrated more optimistic outcomes than the traditional fixed-policy approaches~\cite{rossi2022landing}.

%\begin{figure*}[!tb]
%\begin{center}
%\includegraphics[width=0.8\textwidth]{figures/AI_for_network}
%\caption{AI/ML for network management: An example.}\vspace{-0.6cm}
%\label{fig:ai_for_networking}
%\end{center}
%\end{figure*}

Despite the enormous interest, AI/ML is still immature for deployment in real networks. According to a recent report~\cite{ava}, $88\%$ of the telco industry's proof-of-concept AI/ML projects fail to reach live deployment. The major deterrent stems from inadequate ``system thinking''. %as researchers are not always exposed to the complexities of production networks~\cite{sculley2015hidden}. 
Based on our observation, existing AI/ML-based solutions have two fundamental disparities with real-network deployments: (i) {\em One-dimensional design:} ML solutions mainly aim to outperform prior solutions on specific metrics, especially accuracy, without vetting other network-/system-critical imperatives. For example, %as networks usually operate at very high speeds, it is arduous to obtain high-quality data and features~\cite{bronzino2021traffic}; 
as networks usually become increasingly complex and intertwined, optimization becomes multi-metric and multi-dimensional.
(ii) {\em System discrepancy:} These solutions were mostly demonstrated in controlled environments and became costly to fit into real network systems with much higher scale, complexity, and dynamism. For instance, given the data-driven nature of ML-based solutions, ensuring their performance under sporadic data drifts and system evolutions is non-trivial~\cite{yang2021quality}.
Consequently, this "reality gap" hampers the integration and deployment of AI/ML in real networks. 

%\QL{It is worth mentioning that a modern technology currently in use is network-oriented Development and Operations (DevOps). Simply put, DevOps is an agile methodology that combines software development (Dev) and IT operations (Ops) to shorten the system development life cycle by offering continuous delivery.}
%It is pertinent to note that a mature technology currently employed is network-oriented Development and Operations (DevOps), which combines software development (Dev) and IT operations (Ops), aiming to condense the system development lifecycle through the facilitation of continuous delivery. 
In information technology (IT) industry, the development and delivery of software products is usually streamlined via Development and Operations (DevOps) practices, which are further customized by the telco industry to enhance service quality and reduce time-to-market~\cite{john2017service}.
Although network-oriented DevOps practices offset part of the exertions via continuous integration and delivery, they can hardly accommodate the unique characteristics of AI/ML~\cite{yang2021quality}. To smoothly {\em operationalize} (i.e., {\em develop}, {\em deploy}, and {\em manage}) AI/ML in production, network operators must master skills in ML, data engineering, and systems, which is extremely burdensome. 

This paper aspires to elucidate the practical challenges of integrating AI/ML into the future network landscape. Specifically, we present network-oriented AI/ML research and its gap with real networks. Then, we enumerate the practical considerations to actualize AI/ML in production-ready networks. Afterward, we prospect a promising direction—Machine Learning Operations (MLOps), which closes the gap of operationalizing AI/ML in telco networks. 

%We believe MLOps can relieve the associated operational overhead by adopting time-tested practices. At the same time, Causal AI navigates a novel path toward verifiable AI via casual reasoning and hypothesis testing. Both will play an important role in the future path to adopting AI/ML for networks.

{\color{blue} Chip Huyen's book \cite{huyen2022designing}.}
